Algorithms in the Stacks: Investigating automated, for-profit diversity audits in public libraries

Algorithmic systems are increasingly being adopted by cultural heritage institutions like libraries. In this study, we investigate U.S. public libraries' adoption of one specific automated tool -- automated collection diversity audits -- which we see as an illuminating case study for broader trends. Typically developed and sold by commercial book distributors, automated diversity audits aim to evaluate how well library collections reflect demographic and thematic diversity. We investigate how these audits function, whether library workers find them useful, and what is at stake when sensitive, normative decisions about representation are outsourced to automated commercial systems. Our analysis draws on an anonymous survey of U.S. public librarians (n=99), interviews with 14 librarians, a sample of purchasing records, and vendor documentation. We find that many library workers view these tools as convenient, time-saving solutions for assessing and diversifying collections under real and increasing constraints. Yet at the same time, the audits often flatten complex identities into standardized categories, fail to reflect local community needs, and further entrench libraries' infrastructural dependence on vendors. We conclude with recommendations for improving collection diversity audits and reflect on the broader implications for public libraries operating at the intersection of AI adoption, escalating anti-DEI backlash, and politically motivated defunding.

==> Tables/Price-DivAudit-Interview.tex <==
\resizebox{\columnwidth}{!}{
\footnotesize
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{lcc}
\toprule
Total Estimated Audit Price                      & Vendor-Driven & In-House \\ \midrule
\textbf{Less than \$1,000  }           & 3\%                                                                                                                                                                                & \textbf{30\% }                                                                                                                                                                      \\
\$1,000–\$4,999               & 15\%                                                                                                                                                                               & 16\%                                                                                                                                                                         \\
\textbf{\$5,000–\$9,999}              & \textbf{28\% }                                                                                                                                                                          \  & 21\%                                                                                                                                                                         \\
\$10,000–\$19,999             & 13\%                                                                                                                                                                               & 2\%                                                                                                                                                                          \\
\$20,000–\$29,999             & 0\%                                                                                                                                                                               & 2\%                                                                                                                                                                          \\
\$30,000 or more              & 8\%                                                                                                                                                                                & 2\%                                                                                                                                                                          \\
I don't know / Not applicable & 33\%                                                                                                                                                                              & 26\%        \\
\bottomrule
\end{tabular}
}

\caption{Amount of money survey respondents estimate their library has spent on vendor-provided or in-house diversity audits, including new items purchased. (\( n = 39, n = 43 \))}

==> outline.tex <==


1. Intro - libraries are conducting diversity audits 
we are able to get a window into government spending 
especially around the libraries 

Diversity audits are an example of new tools that library vendors are offering,
because these companies already have a stranglehold on these companies, 
the rest of what they are buying is very expensive
these are one example of new suite of AI type products that are offered by 
these companies 

Especially with AI there is a flurry of AI tools and services offered to companies, 
non-profits, what are these audits.. paying for services in addition to catalog 

Data Cartels Sara Lambden ... analytics ... 





Research Questions: 




- Who is offering diversity audits 
- What forms do they take
- Do only major players offer them 
- How rare are diversity audits 
- Do they appear to concentrated in specific places 

- Does the purchase of diversity audits maintain or displace existing vendor relationships...
- How does the purchase compare to other purchases form this vendor 
    How much do library typically pay main vendors over the course three years 
        - overdrive and baker and taylor and ingraham 
- Given this gross amount how does this frame the cost of diversity audits 

2. 
Analyses

- table describing for each company that we saw in the table, a description from their website of what this product 
is

- bar chart of the audits how much to each company y-axis is \$ x-ticks for each company 

- map of the us and show dots for where they are 



- Pie chart for each library - St. Louis Columbus - 
- how much are they spending per vendor - top 10 vendors
- what are they spending on per vendor , the description might not be there but we can try and see if we can categorize
- what is the libraries budget each year
- if we have list of titles... could we go to amazon get description... could we describe their vision of diversity
- they don't say what they use to define diversity ... could we figure out if they are using the headings...
how to get subject headings... 


3. Discussion, analysis, implications

4. Literature review 



